Classification of $k$-tangle projections using cascade representation

The paper addresses the $k$-tangle enumeration problem. We introduce a notion of cascade diagram for $k$-tangle projections. An effective enumeration algorithm for projections is proposed based on cascade representation. Tangles projections with up to 12 crossings are tabulated. We provide also pictures of alternating $k$-tangles with 5 crossing or less.

==> table3.tex <==
\begin{center}
\texttt{\scriptsize
\begin{tabular}{|c||r|r|r|r|r|r|r|r|r|r|r|r|}
\multicolumn{13}{r}{\normalfont\footnotesize{\bf Table 3 }
Number of weak equivalence classes in the set $\A_{n,k}$ of alternating tangles
\refstepcounter{table}\label{table3}}\\[1ex]
\hline $k\setminus n$
    & 1 & 2 & 3 & 4 & 5  & 6   & 7      & 8       & 9       & 10         & 11          & 12\\\hline\hline
  2 & 1 & 1 & 2 & 6 & 19 & 71  & 293    & 1\,348  & 6\,568  & 33\,701    & 178\,706    & 973\,085\\
  3 & . & 1 & 2 & 8 & 29 & 138 & 638    & 3\,237  & 16\,805 & 90\,239    & 494\,151    & 2\,756\,453\\
  4 & . & . & 2 & 8 & 41 & 210 & 1\,125 & 6\,138  & 34\,112 & 192\,278   & 1\,096\,560 & 6\,317\,363\\
  5 & . & . & . & 5 & 31 & 231 & 1\,458 & 9\,183  & 56\,084 & 340\,885   & 2\,060\,224 & 12\,446\,400\\
  6 & . & . & . & . & 16 & 161 & 1\,406 & 10\,572 & 74\,331 & 499\,902   & 3\,276\,104 & 21\,112\,641\\
  7 & . & . & . & . & .  & 60  & 840    & 8\,818  & 75\,747 & 591\,091   & 4\,327\,816 & 30\,451\,898\\
  8 & . & . & . & . & .  & .   & 261    & 4\,702  & 56\,199 & 541\,570   & 4\,628\,641 & 36\,633\,417\\
  9 & . & . & . & . & .  & .   & .      & 1\,243  & 26\,753 & 361\,106   & 3\,846\,580 & 35\,758\,786\\
  10& . & . & . & . & .  & .   & .      & .       & 6\,257  & 155\,593   & 2\,332\,512 & 27\,199\,662\\
  11& . & . & . & . & .  & .   & .      & .       & .       & 32\,721    & 916\,595    & 15\,123\,600\\
  12& . & . & . & . & .  & .   & .      & .       & .       & .          & 175\,760    & 5\,464\,661\\
  13& . & . & . & . & .  & .   & .      & .       & .       & .          & .           & 963\,900\\\hline
all & 1 & 2 & 6 & 27& 136& 871 & 6\,021 & 45\,241 & 352\,856& 2\,839\,086& 23\,333\,649& 195\,201\,866\\\hline%\cline{2-12}
\end{tabular}}
\end{center}

